PECAN: Personalizing Robot Behaviors through a Learned Canonical Space

Robots should personalize how they perform tasks to match the needs of individual human users. Today's robot achieve this personalization by asking for the human's feedback in the task space. For example, an autonomous car might show the human two different ways to decelerate at stoplights, and ask the human which of these motions they prefer. This current approach to personalization is indirect: based on the behaviors the human selects (e.g., decelerating slowly), the robot tries to infer their underlying preference (e.g., defensive driving). By contrast, our paper develops a learning and interface-based approach that enables humans to directly indicate their desired style. We do this by learning an abstract, low-dimensional, and continuous canonical space from human demonstration data. Each point in the canonical space corresponds to a different style (e.g., defensive or aggressive driving), and users can directly personalize the robot's behavior by simply clicking on a point. Given the human's selection, the robot then decodes this canonical style across each task in the dataset -- e.g., if the human selects a defensive style, the autonomous car personalizes its behavior to drive defensively when decelerating, passing other cars, or merging onto highways. We refer to our resulting approach as PECAN: Personalizing Robot Behaviors through a Learned Canonical Space. Our simulations and user studies suggest that humans prefer using PECAN to directly personalize robot behavior (particularly when those users become familiar with PECAN), and that users find the learned canonical space to be intuitive and consistent. See videos here: https://youtu.be/wRJpyr23PKI

==> 5_theory.tex <==
\section{Theoretical Analysis}\label{sec:theory}


As mentioned in Section~\ref{sec:method}, our method takes as input a dataset of trajectories $x \in X$ where each trajectory corresponds to a specific task $\tau$ and user style $\phi$. The robot knows the number of tasks and style dimensions but not the specific task or style of any trajectory. Our method tries to capture the task labels of input trajectories using discrete one-hot latent variables and their styles with continuous latent variables.
Here we examine when our method can accurately encode the tasks and the styles of trajectories with the one-hot and continuous latent variables, respectively.

\subsection{Separately encoding tasks and user styles}
% Note: This covers having a one-hot encoded latent space for tasks, and how well our network architecture separates the latent tasks and styles depending on the variance in tasks and styles in the demonstrations. This can also discuss how labels help to separate the tasks and styles even when the variance is unfavorable.

\p{Clustering analogy}
We consider settings with $k$ tasks, $\mathcal{T} = \{\tau_{1}, \ldots, \tau_{k}\}$, and a dataset $X$ containing trajectories of different users in each of the $k$ tasks. Since each user can have a distinct style, $\phi \in \Phi$, they would provide different trajectories in the same task. Let $c_{i}$ be the subset of all user trajectories in task $\tau_{i} \in \mathcal{T}$ and $C = \{c_{1}, \ldots, c_{k}\}$ be the set of all such subsets. 
% We consider that the trajectories in $X$ that belong to the same task form a cluster $c$. Therefore the dataset contains $k$ clusters $C = \{c_{1}, \ldots, c_{k}\}$. The variations in the trajectories within the same cluster represent the different user styles in that task.
We want our task encoder to map all trajectories in the same task to a common value of the one-hot latent variable. Therefore the trajectories in each subset $c_{i} \in C$ should map to a different one-hot value. However, the task encoder does not know the task labels for any of the input trajectories.

This problem is analogous to the unsupervised clustering of trajectories where the one-hot values represent the task labels and the subsets $C$ represent the corresponding clusters. To make this analogy, we modify our proposed architecture to separately encode and decode the latent task information using our task encoder $\mathcal{E}_{\tau}$ and a task decoder $\mathcal{D}_{\tau}: Z_{\tau} \mapsto X$. We train both networks with the following reconstruction loss:
\begin{equation}
    \mathcal{L}_{\tau} = ||X - \hat{X} ||^{2} = ||X - \mathcal{D}_{\tau}(\mathcal{E}_{\tau}(X)) ||^{2} \label{eq:loss_task}
\end{equation}
Regardless of the variation in trajectories in a given task, our task encoder must map them to the same one-hot value. For the same one-hot encoding, the task decoder will output the same trajectory. Thus to minimize $\mathcal{L}_{\tau}$, the output of the task decoder would have to be the average of the trajectories corresponding to the encoded task.
This is equivalent to the objective function of $k$-means clustering.
\begin{equation}
    \min_{\hat{C}} \sum_{i=1}^{k} \sum_{x \in \hat{c}_{i}} ||x - \hat{\mu}_{i}||^{2} \label{eq:cluster}
\end{equation}
Here $\hat{C} = \{\hat{c}_{1}, \ldots, \hat{c}_{k}\}$ is the set of clusters formed by the clustering approach and $\{\hat{\mu}_{1}, \ldots, \hat{\mu}_{k}\}$ are the respective cluster means. With this analogy, we now provide conditions for when the trajectories can be accurately clustered, i.e., encoded using the one-hot latent variables.

\p{Multi-modality criterion} 
To explain our theoretical analysis, we consider a simple setting with $2$-D trajectories in $k=2$ tasks and assume that the variation of trajectories in each task follows a bivariate Gaussian distribution. Let $\mu_{1}, \mu_{2} \in \mathbb{R}^{2}$ be the mean trajectories of each task cluster and $\Sigma_{1}, \Sigma_{2} \in \mathbb{R}^{2\times2}$ be their respective covariances. The distribution of trajectories across both tasks is a mixture $g$ of the individual task distributions $g_{1} \sim \mathcal{N}(\mu_{1}, \Sigma_{1})$ and $g_{2} \sim \mathcal{N}(\mu_{2}, \Sigma_{2})$.
\begin{equation}
    g(x) = p g_{1}(x) + (1-p) g_{2}(x)
\end{equation}
Here $p \in (0, 1)$ is the mixing ratio. We set $p=0.5$ to represent that each task is equally likely to occur in the dataset.

If the two distributions are identical ($\mu_{1} = \mu_{2}$ and $\Sigma_{1} = \Sigma_{2}$) we would not find a unique solution for the clustering objective in Equation~\ref{eq:cluster}. To have distinct task clusters, the means of the two distributions should be farther apart ($\mu_{1} \neq \mu_{2}$). Moreover, we want the task clusters to be separated such that the means learned by the clustering approach match the actual means of the task clusters ($\hat{\mu}_{1} = \mu_{1}$ and $\hat{\mu}_{2} = \mu_{2}$). In other words, the only combination of clusters that minimizes the clustering objective is the actual task clusters ($\hat{C} = C$).

We refer to prior research on the bimodality of $1$-D Gaussian mixtures~\cite{schilling2002human} to provide a formal criterion for the separation between the means of the actual task clusters. Based on their analysis, a mixture of two Gaussians is bimodal if it has a local minimum between the means $\mu_{1}$ and $\mu_{2}$. 
\begin{equation}
    \exists \; x \in (\mu_{1}, \mu_{2}) \quad \text{s.t.} \;\; g'(x) = 0 \;\; \text{and} \;\; g''(x) > 0
\end{equation}

Solving for the local minimum results in the following criterion for the bimodality of 1-D Gaussian mixtures:
\begin{equation}
    |\mu_{2} - \mu_{1}| > S(r)(\sigma_{1} + \sigma_{2}) \label{eq:separate}
\end{equation}
Here $S(r)$ is a separation factor. While the prior research finds $S(r) \leq 1$ in theory, they report that higher values of $S(r)$ are required to ensure bimodality in practice. In our analysis, we choose $S(r) = 2$ to enforce a greater separation between the task distributions.

To apply this criterion in our $2$-D setting, we propose that it is sufficient to ensure the separation of task distributions along the straight line connecting their means. The distance between the means along this line is the shortest distance $||\mu_{2} - \mu_{1}||$. We project the trajectories in each task onto this line,  measure their distance from the respective task means, and compute the standard deviations of the projected distributions. 

\p{Clustering accuracy}
Let $c_{1}$ and $c_{2}$ be the clusters of trajectories from the two task distributions. The criterion presented in Equation~\ref{eq:separate} verifies whether the task clusters in the dataset are well separated. Ideally, every trajectory in a cluster is closer to its mean than the means of the other clusters.
\begin{equation}
    |x - \mu_{i}| < |x - \mu_{j}| \quad \forall \; x \in c_{i} \quad c_{i}, c_{j \neq i} \in C \label{eq:no_overlap}
\end{equation}
% The task encoder $\mathcal{E}_{\tau}$ maps any input trajectory to a discrete one-hot latent variable $z_{\tau}$. Thus it performs a hard clustering of the trajectories and does not output probabilities over the latent task variables. As discussed above, the clusters are formed by minimizing the distance of the trajectories from the cluster means.

However, in reality, the clusters can overlap. If a trajectory in one task, $x \in c_{i}$, is closer to the mean of another task cluster $c_{j}$, the $k$-means objective will not include it in the same cluster as other trajectories in $c_{i}$.
The maximum accuracy $P(C|X)$ of clustering the trajectories in a dataset $X$ can be empirically computed given the actual clusters $C$.
\begin{equation}
    P(C|X) \leq \frac{1}{|C|}\sum_{c_{i} \in C} \frac{1}{|c_{i}|} \sum_{x \in c_{i}} \delta(x)
\end{equation}
\begin{equation}
    \delta = 
    \begin{cases}
        1 & \text{if $|x - \mu_{i}| < |x - \mu_{j\neq i}|$}\\
        0.5 & \text{if $|x - \mu_{i}| = |x - \mu_{j\neq i}|$}\\
        0 & \text{if $|x - \mu_{i}| > |x - \mu_{j\neq i}|$}
    \end{cases}
    \quad \forall c_{j \neq i} \in C
    \label{eq:acc}
\end{equation}

We conduct simulation experiments to validate our proposed criterion (Equation~\ref{eq:separate}) and bounds (Equation~\ref{eq:acc}) for accurately encoding the tasks using the one-hot latent variables.

\subsection{Validation experiment}


%% OLD stuff

% Each trajectory $\xi \in \Xi$ corresponds to a task $\tau \in \mathcal{T}$ and user style $\phi \in \Phi$. Let the dataset contain $|\mathcal{T}| = N$ tasks.
% \begin{equation}
%     P(\xi) = \sum_{k=1}^{N} P(\tau_{k}) \mathcal{N} (\xi | \mu_{k}, \Sigma_{k})
% \end{equation}
% \begin{equation}
%     \mathcal{N} (\xi | \mu_{k}, \Sigma_{k}) = \frac{1}{(2\pi)^{M/2} |\Sigma|^{1/2}} \exp\left(-\frac{1}{2} (\xi-\mu)^{T} \Sigma^{-1} (\xi - \mu)\right)
% \end{equation}

% \textit{Approach:}
% \begin{itemize}
%     \item Fit a Gaussian mixture model directly on the trajectory data or after it has been reduced using PCA.
%     \item Show that this is the lower bound (results look more like an upper bound) for our autoencoder without any labels. Adding labels should result in a better performance.
% \end{itemize}


% \subsection{PAC-Bayes Bounds for CLEAR}

% \p{Analogy} The robot interacts with humans that have different styles $\phi \sim \Phi$. These styles are learned from previous demonstrations. Let us consider that the robot has interacted with $N$ humans such that $\mathcal{S} = \{\phi_{1}, \ldots, \phi_{N}\}$. For every $k$-th human, the robot records their trajectories $\Xi_{k}^{i} = \{\xi_{k}^{1}, \ldots\}$ in different tasks $\tau^{i} \in \mathcal{T}$.

% CLEAR inputs the trajectories $\Xi_{k} = \{\Xi_{k}^{1}, \ldots, \Xi_{k}^{|\mathcal{T}|} \}$ to the task and style encoders and estimates the human's latent style $z_{\phi}$ across tasks $\{z_{\tau}^{1}, \ldots, z_{\tau}^{|\mathcal{T}|}\}$. Generally, the robot starts with a uniform prior over the space of latent styles, $P_{0} = U[-1, 1]^{d}$, and learns a posterior $P(z_{\phi}  | \Xi)$.
% {\color{gray} In our theoretical analysis, we assume the autoencoder has a Gaussian prior $P_{0} = \mathcal{N}(0, 1 | \Xi)$ and outputs a posterior $P(z_{\phi}|\Xi) = \mathcal{N}(\mu, \Sigma | \Xi)$.}
% The trajectory decoder then inputs the latent styles $z_{\phi} \sim P(\cdot|\Xi)$ and reconstructs the human's trajectories $\hat{\Xi}$ for each latent task $z_{\tau}^{i}$.

% Therefore, the robot learns to reproduce the human's trajectories from their latent styles $z_{\phi}$. We let $C(z_{\phi}, \phi) = d(\Xi, \hat{\Xi})$ be the difference between the human's trajectories and those produced by the robot based on $z_{\phi}$. We normalize this cost so that $0 \leq C(z_{\phi}, \phi) \leq 1$.

% \p{Bound} Consider a robot trained with $N$ humans with different styles $\mathcal{S} = \{\phi_{1}, \ldots, \phi_{N}\}$. Let $C_{\mathcal{S}}$ be
% the mean cost of CLEAR across these humans. For any $\delta \in (0, 1)$, with a probability of at least $1 - \delta$, the robot's average cost $C_{\mathcal{P}}$ across the entire distribution of latent styles $\mathcal{P}(\phi)$ is less than:
% \begin{equation}
%     C_{\mathcal{P}}(P) \leq C_{\mathcal{S}}(P) + \sqrt{\frac{\text{KL}(P || P_{0}) + \log(\frac{2\sqrt{N}}{\delta})}{2N}}
% \end{equation}
% Here $\text{KL}(P || P_{0})$ is the Kullback-Leibler divergence between the learned posterior over the latent styles $P(z_{\phi}|\Xi)$ and the prior $P_{0}$. The average cost across the known latent styles is:
% \begin{equation}
%     C_{\mathcal{S}}(P) = \frac{1}{N} \sum_{k=1}^{N} \frac{1}{|\Xi_{k}|} \sum_{\Xi_{k}^{i} \in \Xi_{k}}  \mathbb{E}_{z_{\phi} \sim P(\cdot|\Xi_{k}^{i})} C(z_{\phi}, \phi_{k})
% \end{equation}

% \p{Takeaway} The PAC-Bayes bound is too loose. Increasing the number of training inputs $N > 100$ will make it tighter. However, this would mean that we train our model on demonstrations from more than $100$ humans; which is unreasonable. We posit that this bound will be useful only for complex tasks where generalizing to new data is challenging. We will reconsider the PAC-Bayes bound in more complex tasks.

